Learning from Context or Names? An Empirical Study on Neural Relation Extraction

Neural models have achieved remarkable success on relation extraction (RE) benchmarks. However, there is no clear understanding which type of information affects existing RE models to make decisions and how to further improve the performance of these models. To this end, we empirically study the effect of two main information sources in text: textual context and entity mentions (names). We find that (i) while context is the main source to support the predictions, RE models also heavily rely on the information from entity mentions, most of which is type information, and (ii) existing datasets may leak shallow heuristics via entity mentions and thus contribute to the high performance on RE benchmarks. Based on the analyses, we propose an entity-masked contrastive pre-training framework for RE to gain a deeper understanding on both textual context and type information while avoiding rote memorization of entities or use of superficial cues in mentions. We carry out extensive experiments to support our views, and show that our framework can improve the effectiveness and robustness of neural models in different RE scenarios. All the code and datasets are released at https://github.com/thunlp/RE-Context-or-Names.

==> backup.tex <==
\begin{comment}
\appendix

\section{Appendices}
\label{sec:appendix}

\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{c|c|ccc|ccc}
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{1\%} & \multicolumn{3}{c}{100\%} \\
        & & C+M & OnlyC & OnlyM & C+M & OnlyC & OnlyM \\
        \midrule
        \multirow{3}{*}{NYT10} & BERT & 0.277  & 0.128 & 0.192 &0.459 & 0.195 & 0.330\\
        & MTB & 0.281 & 0.135 & 0.194 & 0.453 &0.197 & 0.333 \\
        & CP & 0.278 & 0.131 & 0.183 &  0.453 & 0.197 & 0.327 \\
    \end{tabular}
    \caption{Results on distant supervision dataset NYT-10.}
    \label{tab:distant-supervised}
\end{table*}



\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{c|c|ccc|ccc}
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{5-way-1-shot} & 
        \multicolumn{3}{c}{5-way-5-shot} \\
        & & C+M & OnlyC & OnlyM & C+M & OnlyC & OnlyM \\
        \midrule
        \multirow{3}{*}{FewRel-1.0} & BERT & 0.911 &0.866& 0.701 &0.946 &0.925 & 0.804\\
        & MTB  & 0.911&0.879&0.727 & 0.954& 0.939&0.835  \\
        & CP  &0.951 &0.926 &0.743 &0.971 &0.956 &0.840 \\
        \midrule
        \multirow{3}{*}{FewRel-2.0~(DA)} & BERT  & 0.746&0.683 &0.316&0.827 &0.782 &0.406\\
        & MTB  & 0.747& 0.692&0.338&0.879 &0.836 &0.426 \\
        & CP  &0.797 &0.745 &0.335&0.849 &0.840 &0.437\\
    \end{tabular}
    \caption{FewShot}
    \label{tab:fewshot5}
\end{table*}



% backup
\begin{table*}[h]
    \small
    \centering
    \begin{tabular}{c|c|ccc|ccc}
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{1\%} & \multicolumn{3}{c}{100\%} \\
        & & C+M & OnlyC & OnlyM & C+M & OnlyC & OnlyM \\
        \midrule
        \multirow{3}{*}{TACRED} & BERT & 0.211  & 0.167 & 0.220 & 0.683 & 0.570 & 0.466\\
        & MTB & 0.304 & 0.231 & 0.308 & 0.691 & 0.581 & 0.433 \\
        & CP & 0.485 & 0.393 & 0.350 &  0.695 & 0.593 & 0.450 \\
        \midrule
        \multirow{3}{*}{SemEval} & BERT & 0.367 & 0.294 & 0.245  & 0.871 & 0.798 & 0.677 \\
        & MTB & 0.362 & 0.330 & 0.249 & 0.873 & 0.807 & 0.682 \\
        & CP & 0.482  & 0.470 & 0.221 & 0.876  & 0.811  & 0.679 \\
        \midrule
        \multirow{3}{*}{Wiki80} & BERT & 0.559 & 0.413 & 0.463  & 0.913 & 0.810 & 0.781\\
        & MTB & 0.585  & 0.509 & 0.542  & 0.916 & 0.820 & 0.788  \\
        & CP & 0.827  & 0.734 & 0.653  & 0.922  & 0.834 & 0.799  \\
        \midrule
        \multirow{3}{*}{ChemProt} & BERT & 0.362  & 0.362 & 0.362  & 0.792  & 0.777 & 0.463 \\
        & MTB & 0.362  & 0.362 & 0.362  & 0.796  & 0.798 & 0.463  \\
        & CP & 0.361 & 0.362 & 0.360  & 0.806  & 0.803 & 0.467  \\
    \end{tabular}
    \caption{Supervised}
    \label{tab:supervised}
\end{table*}


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/CN_vs_OC.pdf}
    \caption{Comparison between C+M and OnlyC settings. Blue bar corresponds F1 of C+M setting and green bar corresponds F1 of OnlyC setting.}
    \label{fig:cn_vs_oc}
\end{figure}

\end{comment}





\begin{comment}
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|l|ccc}
        \toprule
        \textbf{Dataset} & \textbf{Model} & \textbf{C+M} & \textbf{OnlyC} & \textbf{OnlyM} \\
        \midrule
        %\multirow{3}{*}{TACRED} & BERT & 0.683 & 0.570 & 0.466\\
        %& MTB  & 0.691 & 0.581 & 0.433 \\
        %& CP & 0.695 & 0.593 & 0.450 \\
        %\midrule
        \multirow{3}{*}{SemEval} & BERT & 0.871 & 0.798 & 0.677 \\
        & MTB &  0.873 & 0.807 & 0.682 \\
        & CP &  0.876  & 0.811  & 0.679 \\
        \midrule
        \multirow{3}{*}{Wiki80} & BERT   & 0.913 & 0.810 & 0.781\\
        & MTB & 0.916 & 0.820 & 0.788  \\
        & CP &  0.922  & 0.834 & 0.799  \\
        \midrule
        \multirow{3}{*}{ChemProt} & BERT &  0.792  & 0.777 & 0.463 \\
        & MTB &  0.796  & 0.798 & 0.463  \\
        & CP &  0.806  & 0.803 & 0.467  \\
        \bottomrule
    \end{tabular}
    \caption{Results on supervised RE datasets SemEval (micro F$_1$), Wiki80 (accuracy) and ChemProt (micro F$_1$). We can see a similar trend to results in Table~\ref{tab:supervised_tacred}.}
    \label{tab:supervised}
\end{table}
\end{comment}

\begin{comment}
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|ccccc|ccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{$1\%$}} & \multicolumn{5}{c}{\textbf{$100\%$}} \\
    & \textbf{C+M}  & \textbf{C+T} & \textbf{OnlyC} & \textbf{OnlyM} & \textbf{OnlyT} & \textbf{C+M}  & \textbf{C+T} & \textbf{OnlyC} & \textbf{OnlyM} & \textbf{OnlyT} \\
    \midrule
    %CNN  & 0.043 & 0.275 & 0.031 & 0.121 & 0.380 & 0.459 & 0.548 & 0.402 &0.254 & 0.403 \\
    CNN  &0.194 & 0.253 & 0.094 &0.299& 0.353 &0.555 & 0.609& 0.461 &0.450& 0.456 \\
    BERT  & 0.211 & 0.177 & 0.167 & 0.220 & 0.281 & 0.683 & 0.686 & 0.570 & 0.466 & 0.277 \\
    MTB & 0.304 & 0.296 & 0.231 & 0.308 & 0.247 & 0.691 & 0.696 & 0.581 & 0.433 & 0.304 \\
    CP & 0.485 & 0.404 & 0.393 & 0.350 & 0.333 &  0.695 & 0.701 & 0.593 & 0.450 & 0.287 \\
    \bottomrule
    \end{tabular}
    \caption{TACRED results (micro F$_1$) with different models and different settings. ``$1\%$'' and ``$100\%$'' indicate using $1\%$ of the training data and using full training data respectively.}
    \label{tab:supervised_tacred}
\end{table*}
\end{comment}

